SituationAdapt: Contextual UI Optimization in Mixed Reality with Situation Awareness via LLM Reasoning

Mixed Reality is increasingly used in mobile settings beyond controlled home and office spaces. This mobility introduces the need for user interface layouts that adapt to varying contexts. However, existing adaptive systems are designed only for static environments. In this paper, we introduce SituationAdapt, a system that adjusts Mixed Reality UIs to real-world surroundings by considering environmental and social cues in shared settings. Our system consists of perception, reasoning, and optimization modules for UI adaptation. Our perception module identifies objects and individuals around the user, while our reasoning module leverages a Vision-and-Language Model to assess the placement of interactive UI elements. This ensures that adapted layouts do not obstruct relevant environmental cues or interfere with social norms. Our optimization module then generates Mixed Reality interfaces that account for these considerations as well as temporal constraints. For evaluation, we first validate our reasoning module's capability of assessing UI contexts in comparison to human expert users. In an online user study, we then establish SituationAdapt's capability of producing context-aware layouts for Mixed Reality, where it outperformed previous adaptive layout methods. We conclude with a series of applications and scenarios to demonstrate SituationAdapt's versatility.

==> sections/1_introduction_ZL.tex <==
\section{Introduction}

% Mixed Reality (MR) devices are becoming increasingly more mobile, signaling a future where they will be utilized in shared public and private spaces --- ranging from coffee shops and trains to living rooms and offices --- similar to the way tablets and laptops are used today.
% In contrast to these traditional devices, MR UIs transcend device boundaries, seamlessly blending into and overlaying the user's physical surroundings.

Mixed Reality (MR) interfaces have the potential to seamlessly integrate virtual content into physical environments.
This integration offers users flexible access to digital information while maintaining their connection to the physical world.
To bridge the virtual content with the physical world, researchers have been exploring adaptive MR user interfaces, taking into account various factors, including users' cognitive load[], the semantic relationship between virtual and physical worlds, and interaction requirements for virtual elements[]. 
These adaptive MR interfaces normally convert the design and generation of interfaces into an optimization problem which optimizes computational terms, such as visibility, distance, consistency[].

While existing computational adaptive MR interfaces are mostly optimized for single user space, the advent of practical mobile MR devices (Apple Vision pro and Meta Quest Pro) allows users to wear and interact with MR devices in public and shared spaces.
Though several papers explored MR interfaces for collaboration, they focused on the shared interfaces instead of the design of personal interfaces in shared spaces.
This advent requires MR interfaces to be dynamically adapted to changing scenarios within shared environments.
On the other hand, previous studies[] underlined that environmental factors, such as social acceptability, safety, and the functionality of physical object, must be considered and included when designing MR interfaces in shared spaces.
However, these environmental factors are inherently complex influenced by dynamic contexts.
Therefore, it is unclear how to quantify these factors and integrate them into optimization-based adaptive MR user interfaces.

To address this challenge, we propose \projectname, a framework that integrates the suitability of placing virtual elements in physical spaces into the optimization of adaptive MR interfaces.
To estimate the suitability in various environments, we leverage Vision Language Models (VLMs) to understand the context and assess the suitability with appropriate prompts in different contexts.

% design space
\zhipeng{(may not include this section, to be discussed.)}
To understand the environmental factors that affect the interaction experience and performance with virtual elements, we went through the literature on context awareness in Virtual/\allowbreak Augmented/\allowbreak Mixed Reality/\allowbreak (VR/AR/MR/XR) and summarized the contextual factors. 
By categorizing the aspects explored in the literature, we contributed to a design space of environmental factors influencing the suitability of interaction with virtual elements.
We then discussed how these environmental factors are shaped by the physical environment and categorized the interaction with virtual elements from the perspective of input and output. 
Subsequently, we analyzed how the environmental factors affected the suitability of input and output interaction separately.
In doing so, we bridged the context of the physical environment with interaction in MR, aiding in the understanding and estimation of interactions' suitability in various contexts.

% technical evaluation: questionnaire
As the design space suggested that how environmental factors influenced the suitability was complicated, we adopted a top-down method to estimate the suitability in different contexts.
While Vision Language Models (VLMs) demonstrated its capability in understanding images and reasoning about their contents, we employed VLMs to understand the context and rate the suitability of placing virtual elements in different physical spaces.
To validate the efficacy of this approach, we conducted a technical evaluation, comparing VLMs' ratings with participants'.
Based on the established environmental factor space, we designed various scenarios and asked both participants and VLMs to provide suitability rating with exactly same information.
Results indicated that in [xx]\% physical spaces, VLMs achieved comparable ratings to participants.
We further analyzed the scenarios in which VLMs and participants had different opinions and discovered that VLMs might identify details which were ignored by participants and thus provided different ratings.


% Implementation: integrate LLMs with optimization
We then implemented \projectname, which integrated VLMs into an adaptive MR user interface framework to generate interfaces that consider the suitability of the physical environment. 
Taking users' field of view and usable physical spaces as input, \projectname rated the suitability for overlaying and interacting with virtual elements for each physical space. 
Combining the suitability terms and other virtual element-related terms, \projectname outputs an MR interface that is suited to the current physical environment.

% Evaluation
To evaluate the efficacy of \projectname, we conducted a usability study, comparing \projectname with a baseline method which did not take suitability into account.
Results suggested that \projectname could generate interfaces considering the restriction, affordance and social setting of the physical environment. 
We further demonstrate the applicability of \projectname in a series of scenarios with diverse physical context.

In summary, we make the following contributions:

\begin{itemize}
    \item We present \projectname, an adaptive MR user interface technique that leverages the suitability of physical environment for placing virtual elements.
    \item We present a comprehensive contextual factor set for MR interfaces and reveal how the factors affect the suitability of physical spaces. 
    \item We evaluate \projectname compared to a baseline method with a travel planning task in a public space. Participants' feedback illustrated that \projectname made the MR interfaces more appropriate to interact in terms of social acceptability and safe to use.
\end{itemize}






% Mixed Reality (MR) interfaces overlay virtual content onto physical environments, providing sufficient and flexible access to digital information and interaction.
% With the development of MR devices and techniques, users are able to wear them and interact with virtual elements in various contexts, from indoor to outdoor environments[], from being alone to playing with friends[], from productivity to recreation[], etc.
% While MR interfaces seamlessly integrate virtual elements with the physical world, they simultaneously obstruct users' observation and interaction with the occluded physical environment. 
% This occlusion can prompt users to engage in inappropriate behavior, thereby reducing the interaction experience and acceptability of MR devices.

% Considering the following scenario: When a user is wearing an MR device during their flight, overlaying a virtual video player over a non-working seat belt light is acceptable under normal circumstances, but it becomes problematic when visual access to the light is crucial for users. 
% Similarly, while overlaying a video player over the back-seat screens can improve users' experience, placing a virtual browser that the user might interact with beside the user could be socially inappropriate since the user may look at and point to the neighboring passengers.
% Existing adaptive MR user interface techniques primarily consider the requirement of the virtual elements (occlusion[], distance[], visibility[]) and optimize the MR interfaces based on physical objects' semantics[], interaction mobility[], etc., to help users access or interact with the virtual elements. 
% There is a lack of consideration of the suitability of overlaying virtual contents on physical environments.
% As shown in the previous example, the suitability of a physical object varies in different contexts. 
% Thus, it is crucial to have a comprehensive understanding of the context and assess the suitability of physical environments for MR interfaces.

==> sections/2_related_work_ZL.tex <==
\section{Related work}

\subsection{Mixed Reality in Shared Spaces}
% As MR devices are becoming more mobile, it is becoming common and important to use MR in shared spaces.
Given the complicated contextual factors in shared spaces, researchers have been exploring and understanding the contextual factors influencing MR interfaces \cite{grubert2016towards}.
%
As the most direct information about the physical space, physical geometry has been used to place virtual elements. 
\citeauthor{ens2015spatial} took the spatial structure of the physical environment into account and aligned virtual elements with it, including walls, windows, and whiteboards, which sacrifices the functionality of physical objects for the placement of virtual elements \cite{ens2016shared, ens2015spatial}. 
Leveraging the geometric information of the physical space, \citeauthor{lang2019virtual} decided on the best placement and pose of virtual agents \cite{lang2019virtual}, while similarly, \citeauthor{liang2021scene} placed virtual pets in the scene by considering the geometric context \cite{liang2021scene}. 
Beyond the physical surroundings, the specific meaning attributed to the environment is also crucial.
One important and common scenario for using MR in shared spaces is transportation settings \cite{mcgill2020challenges, li2021rear, mcgill2019virtual}. 
\citeauthor{williamson2019planevr} explored the unique challenges and opportunities of using MR within airplane contexts \cite{williamson2019planevr} and suggested that social acceptance and safety must be considered when using VR on an airplane. 
\citeauthor{medeiros2022shielding} further investigated the layout of MR interfaces in shared transit contexts, including vehicles and trains, and concluded several considerations when using VR in shared spaces, including social etiquette, spatial affordance, and safety \cite{medeiros2022shielding}.
Moreover, considering individuals within the shared environment adds another layer of complexity.
\citeauthor{whereputit2022luo} explored a collaboration scenario while both users were wearing on MR devices in a productivity task \cite{whereputit2022luo}.
In this case, the digital elements were shared with each other and their placement should be optimized for both users.
On the other hand, \citeauthor{gugenheimer2017sharevr} explored MR interactions while the user is collaborating with other individuals without a headset \cite{gugenheimer2017sharevr}.
Furthermore, \citeauthor{o2023re} explored the MR interactions with bystanders around the user and their results suggested the need of a socially intelligent bystander awareness system.

While there are multiple factors influencing MR interactions' performance and experience in shared spaces, it is hard to comprehensively model it in a computational manner.
Thus we propose to understand the context from a top-down perspective and reason the priority, requirement, and constraints of MR interactions in shared spaces.


\subsection{Adaptive Mixed Reality (MR) Interfaces}

While MR interfaces integrate virtual elements into the physical environment, they are inherently sensitive to the context.
Therefore, prior works have explored adapting MR interfaces to various factors.

One essential focus of MR adaptive user interfaces is environment-driven adaptation \cite{hettiarachchi2016annexing, jones2014roomalive, niyazov2023user, evangelista2022auit}.
Employing geometry-based approaches, researchers suggested to align virtual contents  with the physical surroundings \cite{du2020depthlab, fender2018optispace, flare2014gal}.
\citeauthor{lages2019walking} dynamically adapted virtual elements to physical windows and walls when the user was walking \cite{lages2019walking}.
\citeauthor{scalar2022qian} adopted a decision-tree-based strategy to adapt AR interfaces to new environments while kept the semantic relationships between virtual and physical elements from the previous layout \cite{scalar2022qian}.
SemanticAdapt included the semantic relationship between virtual and physical objects with other factors such as temporal consistency, occlusion, and proposed an inter programming based optimization approach to obtain the adaptive interface \cite{semanticadapt2022cheng}. 
InteractionAdapt leveraged a similar optimization method but also considered about leveraging physical surfaces to provide haptic feedback for MR interactions \cite{cheng2023interactionadapt}.
On the other hand, \citeauthor{paretooptimal2023johns} proposed a Pareto-optimal method to achieve a balance between competing objectives for MR interface adaptation \cite{paretooptimal2023johns}.
\citeauthor{cho2024minexr} introduced a tool to collect user-defined MR interfaces and analyze them to help researchers gain insights and design new MR interfaces in various contexts \cite{cho2024minexr}.
Other approaches investigated MR interfaces adapted to the user's state and movements \cite{gazeRL2019Gebhardt,visualattentionoptimization2019alghofaili, lu2022exploring, fender2017heatspace, veras2021elbow}.
\citeauthor{contextAwareMR2019lindlbauer} optimized virtual elements' visibility, level of detail and placement based on the estimation of users' cognitive load from pupil dilation \cite{contextAwareMR2019lindlbauer}.
\citeauthor{xrgonomics2021belo}~\cite{xrgonomics2021belo} and \citeauthor{ergo2017maurillo}~\cite{ergo2017maurillo} further optimized virtual interfaces for ergonomics with rule-based estimation \cite{mcatamney1993rula}.

While these adaptive interfaces were designed and implemented in situated scenarios, we aim to adapt MR interfaces to shared spaces and proposed new objective terms that adaptive MR interfaces should consider.
Therefore, we introduced new objective terms and leveraged an existing optimization-based approach and augmented it by integrating AI-based ratings into the objective function.

%Works performing MR UI adaptations based on user state often focus on attention, inferred from eye-tracking data. 
% Several recent works propose performing MR interface adaptations based on user state. %, often leveraging eye-tracking data. 
%For instance, \citeauthor{visualattentionoptimization2019alghofaili}~\cite{visualattentionoptimization2019alghofaili} trained a regression model using eye-tracking for predicting gaze duration. These predictions are then used to optimize the placement of visual elements in the scene.
%\citeauthor{gazeRL2019Gebhardt}~\cite{gazeRL2019Gebhardt}, for instance, used Reinforcement learning to model labeling policies from gaze behavior to support users in a visual search task by filtering unnecessary information.
%\citeauthor{contextAwareMR2019lindlbauer}~\cite{contextAwareMR2019lindlbauer} optimized the visibility, level of detail, and placement of UI elements % in an MR environment 
%based on an estimation of users' cognitive load from pupil dilation. 
%All these works adapt MR virtual contents based on a measure of user attention. 
%While the user state is certainly an important consideration, our work focuses on leveraging the physical affordances of the real world to optimize element placements for interaction.


% The aforementioned prior work either focused exclusively on mid-air interactions~(\cite{xrgonomics2021belo,ergo2017maurillo,spatialconstancy2015ens}) or treated physical objects as mere obstacles and neglects considering how environment features influence interaction~(\cite{semanticadapt2022cheng,scalar2022qian}). 
% % To our understanding, there has also not been an explicit consideration of what interaction techniques are available.
% Furthermore, to our understanding, no prior work explicitly modeled interaction techniques when optimizing UI layouts.
% 's main distinguishing feature from prior UI adaptation approaches, such as \citeauthor{semanticadapt2022cheng}~\cite{semanticadapt2022cheng} and \citeauthor{spatialconstancy2015ens}~\cite{spatialconstancy2015ens}, is its explicit consideration of different interaction modalities.
% Our approach exploits physical environment affordances to optimize element placements that support more ergonomic interaction with different techniques. 


\subsection{LLMs in HCI}

With the impressive performance and developement of Large Language Models (LLMs), applying LLMs in various domains has been widely explored, including writing \cite{chung2022talebrush, gero2022sparks}, learning \cite{baidoo2023education, kung2023performance}, programming \cite{vaithilingam2022expectation, chen2021evaluating, pearce2023examining}.
In HCI community, leveraging LLMs to enhance interaction performance is also a popular topic.
Recent papers explored using LLMs to facilitate information retrieval \cite{jiang2305graphologue}, manage information with multilevel abstraction \cite{suh2023sensecape} and synthesize scholarly literature \cite{kang2023synergi}.

\citeauthor{schmidt2024simulating} introduced that using LLMs to simulate the participants in a survey might obtain artificial answers, but the responses could also be unanticipated and offer insights into potential pitfalls \cite{schmidt2024simulating}.
Though the validity of LLMs' responses are unclear, previous research suggested that responses from public platforms like Prolific and Mechanical Turk were also hard to prove their validity \cite{tang2022replication}.

\citeauthor{hamalainen2023evaluating} explored to compare LLMs' responses to human participants' with a HCI task \cite{hamalainen2023evaluating}.
They leveraged gpt3 to generate open-ended responses about experiencing video games.
Their comparison results suggested that LLMs could produce believable responses.
While it is hard to claim that LLMs could also achieve similar performance in other tasks, this study underscores the potential of LLMs to provide comparable responses about HCI experience.

Therefore, we propose to leverage LLMs to understand the context and reason the suitability of placing virtual element in the current physical space, especially when the space is shared with other individuals, which make the context complicated and hard to be solved by existing approaches.
To validate LLMs' capability in our task, we conducted a survey about context understanding and MR interfaces design and compared LLMs' responses to human ones.


% \subsection{Situated VR Interfaces}
% %While the need for context adaptivity is more a commonly accepted requirement for AR, 
% VR applications have traditionally been designed in a way that isolates users from their surroundings and relies on mid-air free-hand controls.
% However, more recent VR research has also recognized opportunities of situating experiences in physical reality \cite{substitutionalreality2015simeone, realitycheck2019hartmann, cheng2019vroamer, yang2019dreamwalker}.
% %, such as improving immersion \cite{insko2001passive}, task performance \cite{henderson2009opportunistic}, and ergonomics during direct interaction \cite{meier2021tapid, streli2022taptype}.
% Existing approaches situate VR experiences by either visualizing features of the physical environment (\eg~RealityCheck \cite{realitycheck2019hartmann}, Meta Quest's ``bring your own desk'' feature~\cite{oculusdeskintegration}) or co-opting passive affordances in the user's surrounding environment for virtual objects (\eg~Substitutional Reality~\cite{substitutionalreality2015simeone,architect2020lin,knockonwood2020strandholt}).
% \projectName\ takes inspiration from the latter. 
% %Our optimization-based approach automatically lays out the mobile workplace such that a user can employ the most suitable interaction modality for each interface element.
% %represents an alternative approach, where instead of visualizing the physical environment, 
% %Substitutional Reality has been explored at multiple scales, from adapting virtual environments to entire rooms \cite{kinectfusion2011, scalar2022qian} to defining mappings between virtual elements to physical proxies \cite{architect2020lin, knockonwood2020strandholt}. 
% %to enable mobile VR workspaces that facilitate a more productive and ergonomic way of working, we take inspiration from this literature~\cite{substitutionalreality2015simeone}.
% % Specifically, we align user's virtual workspace with the real world by considering the affordances of physical objects that enable ergonomic interactions.

% The surrounding physical environment can both benefit and constrain interactions in VR.
% For instance, physical affordances, especially surfaces, may provide beneficial passive haptic feedback for direct interactions with virtual interfaces \cite{deskbsaedvr2019zielasko, menupassivehaptics2019zielasko, cheng2022comfortable, meier2021tapid, streli2022taptype, fang2023vrhapticsathome, streli2023taplight} (\ie~collocating the virtual interface with the physical surface extends mid-air pointing into on-surface touch). 
% Prior research has shown that direct interaction with virtual elements, particularly when collocated with physical surfaces, improves immersion \cite{insko2001passive, passivefeedbackeffectpresencetaskperformance2010abad}, ergonomics, \cite{deskbsaedvr2019zielasko, menupassivehaptics2019zielasko, cheng2022comfortable, meier2021tapid, streli2022taptype, towardsusablevr1999lindeman} and task performance \cite{henderson2009opportunistic, cheng2022comfortable, passivefeedbackeffectpresencetaskperformance2010abad}.
% %This serves to increase the congruence between physical and virtual spaces, which is highlighted as a factor for productive, safe, healthy and enjoyable virtual workspaces \cite{officeofthefuture2018grubert, practicalvirtualoffices2009ofek}. 
% Beyond providing passive haptic feedback, physical surfaces in the environment may also serve as platforms for more restful and stable interactions~\cite{meier2021tapid, streli2022taptype, veras2021elbow, streli2023taplight}, while supporting users in leveraging their sense of proprioception and kinesthesia~\cite{streli2023hoov,passivepropssurgery1994hinckley}.
% % 
% In our recent study~\cite{cheng2022comfortable}, we demonstrated that element placements aligned with surrounding physical surfaces enable users to adopt more ergonomic postures during interaction (\eg~elbow-rested interaction~\cite{veras2021elbow}). 
% \projectName\ integrates the experimental findings of this study in its optimization model.

% Conversely, 
% % The main caveat to the aforementioned benefits is that 
% interacting around physical objects in VR may result in unintended collisions with the environment, which may not only be distracting but detrimental to a user's safety \cite{semanticadapt2022cheng}. 
% \projectName\ is informed by these empirical insights.
% It aligns a user's virtual workspace with the real world by considering the affordances of physical objects to enable ergonomic interactions while avoiding them if they are obtrusive. 
% %Our approach automatically lays out the mobile workplace
% %such that a user can employ the most suitable interaction modality for each interface element.


